Redundancy Principles for MLLMs Benchmarks

With the rapid iteration of Multi-modality Large Language Models (MLLMs) and the evolving demands of the field, the number of benchmarks produced annually has surged into the hundreds. The rapid growth has inevitably led to significant redundancy among benchmarks. Therefore, it is crucial to take a step back and critically assess the current state of redundancy and propose targeted principles for constructing effective MLLM benchmarks. In this paper, we focus on redundancy from three key perspectives: 1) Redundancy of benchmark capability dimensions, 2) Redundancy in the number of test questions, and 3) Cross-benchmark redundancy within specific domains. Through the comprehensive analysis over hundreds of MLLMs' performance across more than 20 benchmarks, we aim to quantitatively measure the level of redundancy lies in existing MLLM evaluations, provide valuable insights to guide the future development of MLLM benchmarks, and offer strategies to refine and address redundancy issues effectively. The code is available at https://github.com/zzc-1998/Benchmark-Redundancy.

==> sec/0_abstract.tex <==



\begin{abstract}

With the rapid iteration of Multi-modality Large Language Models (MLLMs) and the evolving demands of the field, 
the number of benchmarks produced annually has surged into the hundreds. 
The rapid growth has inevitably led to significant redundancy among benchmarks. 
Therefore, it is crucial to take a step back and critically assess the current state of redundancy and propose targeted principles for constructing effective MLLM benchmarks.
In this paper, we focus on redundancy from three key perspectives:
\textbf{1)} Redundancy of benchmark capability dimensions, 
\textbf{2)} Redundancy in the number of test questions, 
and \textbf{3)} Cross-benchmark redundancy within specific domains.
Through the comprehensive analysis over hundreds of MLLMs' performance across more than 20 benchmarks, 
we aim to quantitatively measure the level of redundancy lies in existing MLLM evaluations, 
provide valuable insights to guide the future development of MLLM benchmarks,
and offer strategies to refine and address redundancy issues effectively.
\end{abstract}

==> sec/1_intro.tex <==
\section{Introduction}
\label{sec:intro}

%% needs a brief intro
% MLLM Benchmark Related Works.

Model Evaluation has always played a crucial role in the development of Multi-modal Large Language Models (MLLMs). 
Benchmarks serve not only as tools for assessing model accuracy but also as catalysts for driving innovation and improvements within the field. 
In recent years, with the rapid advancement of MLLMs, there has been an explosive growth in Visual Question Answering (VQA) Benchmarks. 
In the early stages, traditional model evaluation benchmarks such as GQA~\cite{hudson2019gqa}, VQA-V2~\cite{antol2015vqa}, VizWiz~\cite{bigham2010vizwiz}, and TextVQA~\cite{singh2019towards} are characterized by relatively simple questions and answers, with responses often being a single word. This limits the depth of understanding and reasoning required from the models, making them less effective at evaluating the complex capabilities of modern MLLMs that are expected to handle more nuanced and context-dependent tasks. 
With the emergence of more powerful MLLMs~\cite{achiam2023gpt, team2023gemini, chen2024internvl, wang2024qwen2, li2024llava, liu2024visual}, traditional evaluation frameworks have become inadequate to meet the flexible evaluation requirements of these advanced models. 
In response, a new generation of VQA benchmarks has arisen, such as MMBench~\cite{liu2025mmbench}, MMVet~\cite{yu2023mm}, and MMMU~\cite{yue2024mmmu}.

As MLLMs have rapidly iterated and evolved, their diverse capabilities across various domains have garnered increasing attention. 
This expansion has led to the development of specialized benchmarks tailored to evaluate MLLMs' performance in specific areas, like 
% \textit{General Understanding} MME~\cite{fu2024mmecomprehensiveevaluationbenchmark}, SEEDBench~\cite{li2024seed}, BLINK~\cite{fu2025blink}, and MMStar~\cite{chen2024we},
% \textit{Mathematics Task}, benchmarks such as MathVista~\cite{lu2023mathvista}, MathVerse~\cite{zhang2025mathverse}, MathVision~\cite{wang2024measuring}, and Dynamath~\cite{zou2024dynamath},
% \textit{Optical Character Recognition (OCR)}, benchmarks like OCR-VQA~\cite{mishra2019ocr}, OCRBench~\cite{liu2023hidden}, and DOC-VQA~\cite{mathew2021docvqa},
% General Understanding ~\cite{fu2024mmecomprehensiveevaluationbenchmark,li2024seed,fu2025blink,chen2024we},
Mathematics Task~\cite{lu2023mathvista,zhang2025mathverse,wang2024measuring,zou2024dynamath},
Optical Character Recognition (OCR)~\cite{mishra2019ocr,liu2023hidden,mathew2021docvqa},
Medical Field~\cite{hu2024omnimedvqa}, Remote Sensing~\cite{li2024vrsbench}, Agents~\cite{yang2024gpt4tools}, GUIs~\cite{baechler2024screenai}, and so on.

The rapid proliferation of benchmarks has inevitably introduced significant redundancies, 
with overlapping capabilities being assessed and recurring questions appearing within and across benchmarks. 
Such redundancies create inefficiencies in model evaluation, repeatedly testing similar aspects of MLLM performance without contributing meaningful new insights. 
Additionally, this trend risks overemphasizing certain task types while neglecting others, 
potentially distorting research priorities. 
In this work, we address these challenges through a comprehensive and systematic exploration.



\subsection{Identifying Redundancy }
Redundancy is an intrinsic and multifaceted issue in MLLM benchmarks, appearing in several key forms:

\begin{itemize}
    \item \textbf{Redundancy across dimensions (intra-bench):} Tasks within the same benchmark may evaluate overlapping capabilities of MLLMs, leading to repetitive assessments.
    \item \textbf{Redundancy among instances (intra-bench):} Certain instances closely resemble others, providing minimal additional differentiation or insight for model evaluation.
    \item \textbf{Redundancy across benchmarks within specific domains:} Benchmarks targeting specific domains often exhibit overlapping objectives or scopes, 
    resulting in duplicated efforts across different evaluation sets.
\end{itemize}


\subsection{Ideal Redundancy Principles}

Effective benchmarks should adhere to the following principles regarding redundancy:

\begin{itemize}
    \item \textbf{Independence of dimensions:}  
    Ideal benchmarks should ensure that its dimensions are largely independent, 
    minimizing overlap between them. 
    However, some degree of redundancy may be inevitable when certain capabilities naturally require the interaction of multiple foundational skills,
    and redundancy should be carefully balanced to avoid excessive overlap while ensuring valid evaluation.
    
    \item \textbf{Optimal instance count:}  
    A well-designed benchmark should strike a balance in the number of instances it includes: neither too few nor too many, to ensure reliable and meaningful evaluations without introducing unnecessary redundancies.
    
    \item \textbf{Domain representativeness:}  
    A comprehensive benchmark targeted to a specific domain should meaningfully represent the domain. 
    This may involve some purposeful overlap with other benchmarks within the same domain to reflect shared core capabilities.
\end{itemize}


\subsection{Benifits of Evaluating Redundancy}

Evaluating and addressing redundancy offers several significant benefits, as shown in \cref{fig:redundancy}:

\begin{itemize}
    \item \textbf{Optimizing benchmark design:} \textbf{1).} Determines whether certain dimensions within a benchmark warrant separate assessments or can be consolidated; \textbf{2).} Identifies the minimal and sufficient number of instances required to accurately assess model performance; \textbf{3).} Assesses the necessity of introducing new benchmarks within specific domains.
    
    \item \textbf{Enhancing efficiency in MLLM evaluation:} 
    \textbf{1).} Determines whether a benchmark deviates from the domain's distribution ;
    \textbf{2).}  Identifies the anchor benchmarks required to evaluate model performance within the domain.
\end{itemize}

By systematically addressing redundancy, we not only enhance the principles of benchmark design but also alleviate the resource demands of MLLM evaluation, 
creating a more streamlined and effective evaluation ecosystem. 




==> sec/2_framework.tex <==


\section{Redundancy Framework}
We present a framework for evaluating redundancy among MLLM capabilities, defined as specific tasks within a benchmark.
Our framework is grounded in the following prior assumption: 

\textit{
When evaluating similar capabilities, 
the performance rankings of MLLMs should exhibit strong correlation. 
Conversely, significant differences in these rankings suggest the evaluated capabilities are relatively independent. }

Based on this principle, 
we propose the \textbf{Performance Correlation Redundancy Framework}, 
which quantifies redundancy by measuring the correlation of MLLM performance rankings. 
To ensure robustness and generalization capability, 
we leverage the comprehensive data from VLMEvalKit~\cite{duan2024vlmevalkit}, 
which includes diverse benchmarks and performance results from more than 100 MLLMs.

\subsection{Dimensions Redundancy}

Assume a benchmark consists of a set of dimensions, denoted as \( X = \{X_1, X_2, \ldots, X_m\} \), where each \( X_i \) represents a specific dimension. Let \( N \) denote the number of MLLMs evaluated on these dimensions. For a given dimension \( X_i \), we denote the ranking of the \( N \) MLLMs on this dimension as \( R_i \).
To quantify the redundancy of \( X_i \), we compute the average rank correlation between \( R_i \) and the rankings \( R_j \) of all other dimensions \( X_j \) (\( j \neq i \)). Formally, the redundancy \( \rho(X_i) \) is defined as:

\begin{equation}
    \rho(X_i) = \frac{1}{m-1} \sum_{\substack{j=1 \\ j \neq i}}^m \text{CORR}(R_i, R_j),
\end{equation}
where \( \text{CORR}(R_i, R_j) \) is the correlation coefficient between the rankings \( R_i \) and \( R_j \).
\begin{itemize}
    \item High $\text{CORR}(R_i, R_j)$ values serve as indicators for identifying potentially redundant dimension pairs.
    \item \( \rho(X_i) \) represents the average redundancy level of dimension $X_i$, providing its overall information overlap. 
\end{itemize}

By calculating the redundancy \( \rho(X_i) \) for all dimensions \( X_i \) in the benchmark and averaging these values, we can obtain the overall internal redundancy of the benchmark as well. Formally, the benchmark internal redundancy \( \rho_{BI} \) is defined as:

\begin{equation}
\rho_{BI} = \frac{1}{m} \sum_{i=1}^m \rho(X_i),
\end{equation}
where \( \rho(X_i) \) is the redundancy of the \( i \)-th dimension as previously defined.
This metric reflects the average similarity among all dimensions within the benchmark. A lower \( \rho_{BI} \) suggests that the dimensions are relatively independent and diverse.



\subsection{Instances Redundancy}

Let a benchmark contain \( M \) total instances (\textit{e.g.}, QA pairs). 
To evaluate redundancy, we begin by calculating the MLLM performance rankings obtained over the full set of all \( M \) instances, 
denoted as the ground-truth ranking \( R_{\text{GT}} \).
We then randomly sample a subset of the instances, comprising A\% of the total M, 
and compute the corresponding MLLM rankings, 
denoted as \( R_{\text{sample}} \). 
To quantify the redundancy of the benchmark at a sampling ratio of \( A\% \), 
we calculate the correlation coefficient between \( R_{\text{sample}} \) and \( R_{\text{GT}} \).
This correlation reflects how representative the sampled subset is of the entire benchmark. 
To reduce the effect of randomness, the sampling process is repeated \(T = 100 \) times, 
and the average correlation result is recorded.
We define the instance redundancy of the benchmark at sampling ratio \( A\% \), 
denoted as \( \rho(A\%) \), as follows:

\begin{equation}
    \rho(A\%) = \frac{1}{T} \sum_{1 \le t \le T} \text{CORR}(R_{A\%_{t}}, R_{\text{GT}}),
\end{equation}

where \( R_{A\%_{t}} \) represents the MLLM ranking based on the sampled \( A\% \) instances at the \( t_{th}\) time, 
and \( R_{\text{GT}} \) is the MLLM ranking based on the full \( M \) instances within the MLLM benchmark. 
The interpretation of \( \rho(A\%) \) is straightforward: 

\begin{itemize}
\item A higher \( \rho(A\%) \) indicates that the sampled instances are highly representative of the entire benchmark, 
and the remaining \( 1-A\%\) instances contribute little additional information, indicating redundancy.
\item Conversely, a lower \( \rho(A\%) \) suggests that the sampled instances are less representative, 
and a larger sample is needed to capture the variability of the full benchmark.
\end{itemize}

% This metric helps determine the proportion of instances sufficient to accurately evaluate the performance of the corresponding MLLMs, significantly reducing the workload required for MLLM evaluation.

\begin{figure}[tbp]
    \centering
    \includegraphics[width=0.85\linewidth]{figs/spotlight.pdf}
    \caption{A quick look at the redundancy framework, where (a), (b), and (c) show the general process of computing dimensions redundancy, instances redundancy, and cross-benchmark redundancy respectively.}
    \label{fig:framework}
\end{figure}

% \begin{figure*}[tbp]
%     \centering
%     \begin{subfigure}[b]{.49\linewidth} 
%         \centering
%         \includegraphics[width=.95\linewidth]{MMB_figs/MMBench_TEST_EN_V11_SRCC_50_heatmap.pdf}
%         \caption{Top-50 SRCC dimensions redundancy map.}
%         \label{fig:MMBench_SRCC_50_heat}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[b]{.49\linewidth}  
%         \centering
%         \includegraphics[width=.95\linewidth]{MMB_figs/MMBench_TEST_EN_V11_SRCC_-50_heatmap.pdf}
%         \caption{Bottom-50 SRCC dimensions redundancy map.}
%         \label{fig:MMBench_SRCC_-50_heat}
%     \end{subfigure}
%     \begin{subfigure}[b]{.49\linewidth} 
%         \centering
%         \includegraphics[width=.95\linewidth]{MMB_figs/MMBench_TEST_EN_V11_PLCC_50_heatmap.pdf}
%         \caption{Top-50 PLCC dimensions redundancy map.}
%         \label{fig:MMBench_PLCC_50_heat}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[b]{.49\linewidth}  
%         \centering
%         \includegraphics[width=.95\linewidth]{MMB_figs/MMBench_TEST_EN_V11_PLCC_-50_heatmap.pdf}
%         \caption{Bottom-50 PLCC dimensions redundancy map.}
%         \label{fig:MMBench_PLCC_-50_heat}
%     \end{subfigure}
%     \begin{subfigure}[b]{.49\linewidth} 
%         \centering
%         \includegraphics[width=.95\linewidth]{MMB_figs/MMBench_TEST_EN_V11_R2_50_heatmap.pdf}
%         \caption{Top-50 R2 dimensions redundancy map.}
%         \label{fig:MMBench_R2_50_heat}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[b]{.49\linewidth}  
%         \centering
%         \includegraphics[width=.95\linewidth]{MMB_figs/MMBench_TEST_EN_V11_R2_-50_heatmap.pdf}
%         \caption{Bottom-50 R2 dimensions redundancy map.}
%         \label{fig:MMBench_R2_-50_heat}
%     \end{subfigure}
%     \caption{Visualizations of dimensions redundancy for MMBench~\cite{liu2025mmbench} on Top-50 and Bottom-50 MLLMs.}
%     \label{fig:MMbench_heat}
% \end{figure*}

\begin{figure*}[tbp]
    \centering
    \begin{subfigure}[b]{.33\linewidth} 
        \centering
        \includegraphics[width=.95\linewidth]{MMB_figs/MMBench_TEST_EN_V11_SRCC_50_heatmap.pdf}
        \caption{Top-50 SRCC dimensions redundancy map.}
        \label{fig:MMBench_SRCC_50_heat}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{.33\linewidth} 
        \centering
        \includegraphics[width=.95\linewidth]{MMB_figs/MMBench_TEST_EN_V11_PLCC_50_heatmap.pdf}
        \caption{Top-50 PLCC dimensions redundancy map.}
        \label{fig:MMBench_PLCC_50_heat}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{.33\linewidth} 
        \centering
        \includegraphics[width=.95\linewidth]{MMB_figs/MMBench_TEST_EN_V11_R2_50_heatmap.pdf}
        \caption{Top-50 R2 dimensions redundancy map.}
        \label{fig:MMBench_R2_50_heat}
    \end{subfigure}
    \begin{subfigure}[b]{.33\linewidth}  
        \centering
        \includegraphics[width=.95\linewidth]{MMB_figs/MMBench_TEST_EN_V11_SRCC_-50_heatmap.pdf}
        \caption{Bottom-50 SRCC dimensions redundancy map.}
        \label{fig:MMBench_SRCC_-50_heat}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{.33\linewidth}  
        \centering
        \includegraphics[width=.95\linewidth]{MMB_figs/MMBench_TEST_EN_V11_PLCC_-50_heatmap.pdf}
        \caption{Bottom-50 PLCC dimensions redundancy map.}
        \label{fig:MMBench_PLCC_-50_heat}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{.33\linewidth}  
        \centering
        \includegraphics[width=.95\linewidth]{MMB_figs/MMBench_TEST_EN_V11_R2_-50_heatmap.pdf}
        \caption{Bottom-50 R2 dimensions redundancy map.}
        \label{fig:MMBench_R2_-50_heat}
    \end{subfigure}
    \caption{Visualizations of dimensions redundancy for MMBench~\cite{liu2025mmbench} on Top-50 and Bottom-50 MLLMs.}
    \label{fig:MMbench_heat}
\end{figure*}


\begin{figure*}[tbp]
    \centering
    \begin{subfigure}[b]{.32\linewidth} 
        \centering
        \includegraphics[width=.95\linewidth]{MMB_figs/MMBench_TEST_EN_V11_SRCC_50_avg_similarity_barplot.pdf}
        \caption{Top-50 SRCC redundancy.}
        \label{fig:MMBench_SRCC_50_bar}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{.32\linewidth}  
        \centering
        \includegraphics[width=.95\linewidth]{MMB_figs/MMBench_TEST_EN_V11_PLCC_50_avg_similarity_barplot.pdf}
        \caption{Top-50 PLCC redundancy.}
        \label{fig:MMBench_PLCC_50_bar}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{.32\linewidth}  
        \centering
        \includegraphics[width=.95\linewidth]{MMB_figs/MMBench_TEST_EN_V11_R2_50_avg_similarity_barplot.pdf}
        \caption{Top-50 R2 redundancy.}
        \label{fig:MMBench_R2_50_bar}
    \end{subfigure}
    \begin{subfigure}[b]{.32\linewidth} 
        \centering
        \includegraphics[width=.95\linewidth]{MMB_figs/MMBench_TEST_EN_V11_SRCC_-50_avg_similarity_barplot.pdf}
        \caption{Bottom-50 SRCC redundancy.}
        \label{fig:MMBench_SRCC_-50_bar}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{.32\linewidth}  
        \centering
        \includegraphics[width=.95\linewidth]{MMB_figs/MMBench_TEST_EN_V11_PLCC_-50_avg_similarity_barplot.pdf}
        \caption{Bottom-50 PLCC redundancy.}
        \label{fig:MMBench_PLCC_-50_bar}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{.32\linewidth}  
        \centering
        \includegraphics[width=.95\linewidth]{MMB_figs/MMBench_TEST_EN_V11_R2_-50_avg_similarity_barplot.pdf}
        \caption{Bottom-50 R2 redundancy.}
        \label{fig:MMBench_R2_-50_bar}
    \end{subfigure}
    \caption{Bar plots of dimensions redundancy for MMBench~\cite{liu2025mmbench} on Top-50 and Bottom-50 MLLMs. The redundancy values are computed by averaging the redundancy of each dimension with the redundancy of all other dimensions.}
    \label{fig:MMbench_bar}
\end{figure*}



% \begin{figure*}[tbp]
%     \centering
%     \begin{subfigure}[b]{.49\linewidth} 
%         \centering
%         \includegraphics[width=\linewidth]{figs/MMBench_TEST_EN_V11_SRCC_50_heatmap.pdf}
%         \caption{Dimensions redundancy map on SRCC.}
%         \label{fig:MMBench_SRCC_50}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[b]{.49\linewidth}  
%         \centering
%         \includegraphics[width=\linewidth]{figs/MMBench_TEST_EN_V11_PLCC_50_heatmap.pdf}
%         \caption{Dimensions redundancy map on PLCC.}
%         \label{fig:MMBench_PLCC_50}
%     \end{subfigure}
%      \vspace{1em} % 增加两行之间的垂直间距
%     \hspace{-0.7cm} % 左移第二行第一张图
%     \begin{subfigure}[b]{.49\linewidth} 
%         \centering
%         \includegraphics[width=.9\linewidth]{figs/MMBench_TEST_EN_V11_SRCC_50_avg_similarity_barplot.pdf}
%         \caption{Average SRCC redundancy.}
%         \label{fig:MMBench_SRCC_50_bar}
%     \end{subfigure}
%     \hspace{0.3cm}
%     \begin{subfigure}[b]{.49\linewidth}  
%         \centering
%         \includegraphics[width=.9\linewidth]{figs/MMBench_TEST_EN_V11_PLCC_50_avg_similarity_barplot.pdf}
%         \caption{Average PLCC redundancy.}
%         \label{fig:MMBench_PLCC_50_bar}
%     \end{subfigure}
%     \caption{Visualizations of dimensions redundancy for MMBench on Top-50 MLLMs.}
%     \label{fig:MMbench_50}
% \end{figure*}


% \begin{figure*}[tbp]
%     \centering
%     \begin{subfigure}[b]{.49\linewidth} 
%         \centering
%         \includegraphics[width=\linewidth]{figs/MMBench_TEST_EN_V11_SRCC_-50_heatmap.pdf}
%         \caption{Dimensions redundancy map on SRCC.}
%         \label{fig:MMBench_SRCC_-50}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[b]{.49\linewidth}  
%         \centering
%         \includegraphics[width=\linewidth]{figs/MMBench_TEST_EN_V11_PLCC_-50_heatmap.pdf}
%         \caption{Dimensions redundancy map on PLCC.}
%         \label{fig:MMBench_PLCC_-50}
%     \end{subfigure}
%      \vspace{1em} % 增加两行之间的垂直间距
%     \hspace{-0.7cm} % 左移第二行第一张图
%     \begin{subfigure}[b]{.49\linewidth} 
%         \centering
%         \includegraphics[width=.9\linewidth]{figs/MMBench_TEST_EN_V11_SRCC_-50_avg_similarity_barplot.pdf}
%         \caption{Average SRCC redundancy.}
%         \label{fig:MMBench_SRCC_-50_bar}
%     \end{subfigure}
%     \hspace{0.3cm}
%     \begin{subfigure}[b]{.49\linewidth}  
%         \centering
%         \includegraphics[width=.9\linewidth]{figs/MMBench_TEST_EN_V11_PLCC_-50_avg_similarity_barplot.pdf}
%         \caption{Average PLCC redundancy.}
%         \label{fig:MMBench_PLCC_-50_bar}
%     \end{subfigure}
%     \caption{Visualizations of dimensions redundancy for MMBench on Bottom-50 MLLMs.}
%     \label{fig:MMbench_-50}
% \end{figure*}



\subsection{Cross-Benchmark Redundancy}
\label{sec2.3}
Consider \( Y = \{Y_1, Y_2, \ldots, Y_l\} \), 
a collection of \( l \) benchmarks within a specific domain
(\textit{e.g.}, object hallucination, visual reasoning, visual perception). 
Let \( N \) represent the number of MLLMs evaluated across these benchmarks. 
For a given benchmark \( Y_i \), 
let \( K_i \) denote the ranking of the \( N \) MLLMs based on their performance on \( Y_i \). 
To identify key anchor benchmarks within this domain 
(an anchor benchmark can serve as a representative over multiple other benchmarks),  
we focus on selecting benchmarks that demonstrate high redundancy with other benchmarks in the domain~\cite{zohar2024apollo}.
We define the redundancy of a benchmark \( \rho(Y_i) \) as the average rank correlation coefficient between \( K_i \) and the rankings \( K_j \) of all other benchmarks \( Y_j \) (\( j \neq i \)) in the domain. 
Formally, \( \rho(Y_i) \) is expressed as:

\begin{equation}
   \rho(Y_i) = \frac{1}{l-1} \sum_{\substack{j=1 \\ j \neq i}}^l \text{CORR}(K_i, K_j), 
\end{equation}
where \( \text{CORR}(K_i, K_j) \) is the correlation coefficient between the rankings \( K_i \) and \( K_j \). 
The interpretation of \( \rho(Y_i) \) is as follows:

\begin{itemize}
    \item A higher \( \rho(Y_i) \) indicates that benchmark \( Y_i \) exhibits strong similarity with other benchmarks in the domain, 
    suggesting that it is highly representative of the domain’s capabilities or evaluation focus.
    \item Conversely, a lower \( \rho(Y_i) \) indicates that benchmark \( Y_i \) shares less overlap with other benchmarks, implying that it is less redundant and may capture unique / distinct aspects of the domain, or incorporate noises which are not related to the domain.
\end{itemize}
% This metric helps in identifying benchmarks that best capture the core characteristics of the domain, facilitating the selection of a reduced yet representative subset of benchmarks.

\subsection{Correlation Metrics}
In this work, we adopt multiple metrics to describe the correlation between two set of performance numbers, 
including the Spearman Rank Correlation Coefficient (SRCC), 
the Pearson Linear Correlation Coefficient (PLCC), 
and the R² Score (R-squared Coefficient of Determination).
\begin{itemize}
\item \textbf{SRCC} is an evaluation metric that measures rank similarity, capturing how well the relative order between two rankings aligns.
\item \textbf{PLCC} quantifies linear similarity, assessing how closely the rankings follow a linear relationship.
\item \textbf{R² Score}, on the other hand, evaluates the proportion of variance explained by the ranking relationship, serving as a measure of goodness-of-fit.
\end{itemize}

\subsection{Top-K Analysis}

Considering that the performance of top-tier MLLMs often garners greater attention on benchmarks, 
we can streamline the redundancy analysis by focusing only on the top-K MLLMs with the highest overall performance on a given benchmark, 
rather than incorporating all MLLMs in the calculation. 
By selecting the top-K models, we can better target the analysis of benchmark redundancy across different performance tiers. 
This approach also simplifies the process of maintaining and updating our framework as new MLLMs are introduced.


==> sec/3_experiment.tex <==


\section{Experiment \& Discussion}

We use the evaluation results of hundreds of MLLMs obtained through the VLMEvalKit~\cite{duan2024vlmevalkit} as our data source 
for conducting experiments and analysis. 
All the data sources we used have been open-sourced on HuggingFace \footnote{\url{https://huggingface.co/datasets/VLMEval/OpenVLMRecords}}.

% \subsection{Data Source}

% All the benchmark performance results come from the OpenCompass platform, which includes over xxx popular benchmarks and xxx MLLMs. 

\subsection{Exploring Dimension Redundancy}

% \subsubsection{BLINK}

% To highlight the differences among dimensions, we specifically select the BLINK Benchmark~\cite{fu2024blink} as our case study. BLINK is known for its diversity and the rich variety of its dimensions. Based on the ranking performance comparison of 177 MLLMs across 13 dimensions on OpenCompass, we create a redundancy heatmap for BLINK's dimensions in Fig.\ref{fig:blink_heatmap}. 

% From the heatmap, we observe that tasks such as \textit{Counting} exhibit a relatively high degree of correlation with \textit{Relative Depth} and \textit{Spatial Relation}. This indicates that models achieving high performance on \textit{Counting} tend to perform well on these dimensions too, suggesting overlapping capabilities in reasoning about quantities, spatial arrangements, and depth perception, which aligns with intuitive expectations. These dimensions likely require similar cognitive mechanisms, such as an understanding of numerical relationships and spatial hierarchies.
% In contrast, the \textit{IQ Test} dimension demonstrates consistently low similarity with all other dimensions. This finding suggests that \textit{IQ Test} is more independent and captures unique aspects of model reasoning or problem-solving capabilities. This independence could imply that the skills required to perform well on \textit{IQ Test} are distinct, such as abstract reasoning, logic, or pattern recognition, which do not overlap significantly with the more perceptual or spatial skills associated with other tasks. This insight emphasizes the need for specialized evaluation metrics for such tasks, as they might provide complementary perspectives on model performance.




\begin{figure*}[tbp]
    \centering
    \begin{subfigure}[b]{.48\linewidth}  % Adjust width to fit side by side
        \centering
        \includegraphics[width=\linewidth]{instance_num_figs/50_metrics_plot.pdf}
        \caption{Instances redundancy with Top-50 MLLMs.}
        \label{fig:instances_top50}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{.48\linewidth}  % Ensure both subfigures are the same width
        \centering
        \includegraphics[width=\linewidth]{instance_num_figs/-50_metrics_plot.pdf}
        \caption{Instances redundancy with Bottom-50 MLLMs.}
        \label{fig:instances_back50}
    \end{subfigure}
    \caption{Visualizations of average instance redundancy for (a) Top-50 MLLMs and (b) Bottom-50 MLLMs across 18 LMM benchmarks (A-Bench~\cite{zhang2024bench}, AI2D~\cite{kembhavi2016diagram}, BLINK~\cite{fu2025blink},  HallusionBench~\cite{guan2023hallusionbench}, MMBench~\cite{liu2025mmbench}, MMMU~\cite{yue2024mmmu}, MME~\cite{fu2024mmecomprehensiveevaluationbenchmark}, MMStar~\cite{chen2024mmstar}, MMT~\cite{ying2024mmt}, MMVet~\cite{yu2023mmvet}, OCRBench~\cite{liu2023ocrbench}, Q-Bench~\cite{wu2023qbench,zhang2024q+}, R-Bench-Dis~\cite{li2024rbench}, RealWorldQA~\cite{RealWorldQA}, ScienceQA~\cite{lu2022learn}, SeedBench\_IMG~\cite{li2023seedimg}, SeedBench2\_Plus~\cite{li2024seed2plus}). Notably, each data point represents the average of 100 sampling iterations to mitigate the impact of randomness. }
    \label{fig:instances_overall}
    \vspace{-0.2cm}
\end{figure*}



To comprehensively demonstrate the application of our redundancy framework in MLLM benchmarks, 
we conduct a detailed case study using the widely adopted and dimensionally diverse MMBench benchmark (v1.1)~\cite{liu2025mmbench}. 
We categorize the MLLMs into two groups, Top-50 and Bottom-50, based on their overall performance in MMBench. 
This categorization enables us to highlight the differences in redundancy exhibited by MMBench when evaluating MLLMs with varying levels of capability. 
The results for the Top-50 and Bottom-50 groups are illustrated in \cref{fig:MMbench_heat} and \cref{fig:MMbench_bar}, respectively, 
from which we derived several interesting insights.


% We exclude the R² Score from the analysis as it measures the fit between two sub-dimensions, and differences in scale between sub-dimensions can lead to significant bias in the results. 
% Additionally, we categorize the MLLMs into Top-50 and Bottom-50 groups based on their overall performance in MMBench (the top 50 and bottom 50 models, respectively). This categorization allows us to highlight the differences in redundancy exhibited by MMBench when evaluating MLLMs with varying capabilities. The results for the Top-50 and Bottom-50 groups are shown in Fig.\ref{fig:MMbench_heat} and Fig.\ref{fig:MMbench_bar}, respectively, from which we derived several interesting insights.

\noindent
\textbf{Top-50 Redundancy. }
\cref{fig:MMBench_SRCC_50_heat,fig:MMBench_PLCC_50_heat} visually illustrate the redundancy of SRCC and PLCC across various sub-dimensions,
allowing for a quick analysis of which dimensions exhibit high correlations. 
For example, the tasks \textbf{Image Emotion} and \textbf{Social Relation} display strong redundancy, suggesting a significant overlap in the skills they assess.
Similarly, \textbf{Structuralized Image-Text Understanding} demonstrates notable redundancy with several other dimensions, such as \textbf{Spatial Relationship}, \textbf{Physical Property Reasoning}, \textbf{OCR}, and \textbf{Nature Relation}, 
indicating that these tasks collectively represent the diverse abilities required to perform \textbf{Structuralized Image-Text Understanding}. 
In contrast, \textbf{Image Topic} and \textbf{Image Scene} exhibit relatively low redundancy with other dimensions, as shown in \cref{fig:MMBench_SRCC_50_bar,fig:MMBench_PLCC_50_bar,fig:MMBench_R2_50_bar}. 
This could arise from the inherent complexity of assessing the overall topic and scene of an image, 
which is often less correlated with evaluating specific attributes or relationships.
For instance, strong performance in recognizing individual attributes does not necessarily imply a comprehensive understanding of the overall topic or scene. 
However, \cref{fig:MMBench_PLCC_50_heat} reveals that these two dimensions exhibit redundancy in terms of PLCC, suggesting potential overlaps within certain contexts.
Another interesting insight arises from \textbf{Celebrity Recognition}, 
a knowledge-based task that remains relatively independent of other dimensions, 
which primarily measure perceptual abilities. 
As a result, it consistently exhibits significantly lower redundancy across SRCC, PLCC, and R². 
Conversely, high levels of redundancy are observed for Nature Relation and Spatial Relationship, as shown in \cref{fig:MMBench_SRCC_50_bar,fig:MMBench_PLCC_50_bar,fig:MMBench_R2_50_bar}. 
This is attributed to the fact that these two dimensions serve as fundamental skills required by numerous other tasks, making their overlap a cornerstone of the broader evaluation framework.

% 2) In contrast, simpler foundational tasks such as \textit{Spatial Relationship}, \textit{Attribute Comparison}, and \textit{Nature Relation} cover a broader range of capabilities and are more closely related to other tasks, leading to higher redundancy. These dimensions often require general-purpose reasoning skills that overlap significantly across tasks.
% 3) Tasks like \textit{Action Recognition}, \textit{Celebrity Recognition}, and \textit{Social Relation} require more specialized knowledge or expertise that may not directly correlate with general capabilities. As a result, these tasks typically exhibit lower redundancy.
% Overall, the analysis suggests that simpler tasks with broader coverage tend to exhibit higher scores and greater redundancy. Conversely, more complex or knowledge-intensive tasks demonstrate lower redundancy, highlighting their distinct and specialized evaluation focus.


\noindent
\textbf{Bottom-50 Redundancy. }
The results for the Bottom-50 redundancy, as shown in \cref{fig:MMBench_SRCC_-50_bar,fig:MMBench_PLCC_-50_bar,fig:MMBench_R2_-50_bar}, 
reveal a striking trend where nearly all dimensions exhibit significantly higher redundancy compared to the Top-50 redundancy. 
Specifically, most dimension pairs achieve SRCC and PLCC scores exceeding 0.6
(\cref{fig:MMBench_SRCC_-50_bar,fig:MMBench_PLCC_-50_bar}), 
leading to an interesting conclusion:
\textbf{the dimensions appear to be more redundant for Bottom-50 MLLMs than for Top-50 MLLMs}.
This phenomenon can primarily be attributed to the fact that Bottom-50 MLLMs generally underperform across all capabilities. 
For these models, as their foundational abilities improve, incremental enhancements in one dimension often drive simultaneous improvements across others. 
This results in high consistency in performance rankings across dimensions, thereby causing relatively high dimensional redundancy.
In contrast, the Top-50 MLLMs have already achieved relatively strong foundational capabilities. 
Consequently, more complex tasks across different dimensions introduce greater variability, allowing for more differentiation between performance in those dimensions. 
This leads to noticeably lower levels of redundancy for the Top-50 models. 
These findings emphasize the importance of carefully selecting the MLLMs included in redundancy analysis. 
Specifically, avoiding models with universally poor performance is crucial to ensure that the evaluation yields meaningful and accurate insights.


\begin{figure*}[tbp]
    \centering
    \begin{subfigure}[b]{.32\linewidth}  % Adjust width to fit side by side
        \centering
        \includegraphics[width=\linewidth]{instance_num_figs/50_SRCC_plot.pdf}
        \caption{Top-50 SRCC redundancy.}
        \label{fig:instances_50_SRCC}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{.32\linewidth}  % Ensure both subfigures are the same width
        \centering
        \includegraphics[width=\linewidth]{instance_num_figs/50_PLCC_plot.pdf}
        \caption{Top-50 PLCC redundancy.}
        \label{fig:instances_50_PLCC}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{.32\linewidth}  % Adjust width to fit side by side
        \centering
        \includegraphics[width=\linewidth]{instance_num_figs/50_R2_plot.pdf}
        \caption{Top-50 R2 redundancy.}
        \label{fig:instances_50_R2}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{.32\linewidth}  % Ensure both subfigures are the same width
        \centering
        \includegraphics[width=\linewidth]{instance_num_figs/-50_SRCC_plot.pdf}
        \caption{Bottom-50 SRCC redundancy.}
        \label{fig:instances_-50_SRCC}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{.32\linewidth}  % Adjust width to fit side by side
        \centering
        \includegraphics[width=\linewidth]{instance_num_figs/-50_PLCC_plot.pdf}
        \caption{Bottom-50 PLCC redundancy.}
        \label{fig:instances_-50_PLCC}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{.32\linewidth}  % Ensure both subfigures are the same width
        \centering
        \includegraphics[width=\linewidth]{instance_num_figs/-50_R2_plot.pdf}
        \caption{Bottom-50 R2 redundancy.}
        \label{fig:instances_-50_R2}
    \end{subfigure}
    \caption{Benchmark-specific instance redundancy for (a) Top-50 MLLMs and (b) Bottom-50 MLLMs. The benchmarks include BLINK~\cite{fu2025blink}, ScienceQA~\cite{lu2022learn}, MMMU~\cite{yue2024mmmu}, RealWorldQA~\cite{RealWorldQA}, MMBench~\cite{liu2025mmbench}, MMStar~\cite{chen2024mmstar}, SeedBench\_IMG~\cite{li2023seedimg}, and AI2D~\cite{kembhavi2016diagram}. The selection of the Top-50 and Bottom-50 MLLMs is based on the corresponding benchmark.}
    \label{fig:instances_bench}
    \vspace{-0.2cm}
\end{figure*}

\begin{figure*}
    \centering
    \includegraphics[width=\linewidth]{figs/appd_mathvista.pdf}
    \caption{Examples of tasks excluded from the MathVista benchmark. (a), (b), and (c) showcase tasks derived from the \textit{general-vqa} category, including \textit{Scientific Figure Understanding}, \textit{General VQA}, and \textit{Chart/Table/Diagram QA}. Panel (d) presents questions extracted from the CLEVR dataset but categorized as \textit{math-targeted-vqa}.}
    \label{fig:append_mathvista}
\end{figure*}

%\subsubsection{CCBench}
% Additionally, we include an analysis of the dimension redundancy in the CCBench benchmark as shown in Fig. \ref{fig:ccbench_heatmap}. It is evident that the dimensions of CCBench exhibit significantly higher redundancy compared to those of BLINK. Notably, the \textit{Cultural Relic} dimension demonstrates exceptionally high similarity with almost all other cultural dimensions. This can be attributed to the nature of CCBench, which is designed as a benchmark focused on knowledge evaluation. As a result, the differences in capability tests among its dimensions are relatively minor. MLLMs with a comparable level of Chinese cultural knowledge tend to exhibit similar performance across these dimensions.
% This observation does not imply that CCBench is a poor benchmark. Instead, it can be understood as an intentional evaluation of MLLMs} diverse knowledge areas using similar capabilities. However, it does validate the effectiveness of our proposed redundancy framework, which proves to be a valuable tool in assessing the redundancy of benchmark dimensions. 

% \begin{figure*}[tbp]
%     \centering
%     \begin{subfigure}[b]{.48\linewidth}  % Adjust width to fit side by side
%         \centering
%         \includegraphics[width=\linewidth]{figs/top50_metrics_plot.pdf}
%         \caption{Instances redundancy with sampling percentage.}
%         \label{fig:instances_percentage}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[b]{.48\linewidth}  % Ensure both subfigures are the same width
%         \centering
%         \includegraphics[width=\linewidth]{figs/back50_metrics_plot.pdf}
%         \caption{Instances redundancy with sampling number.}
%         \label{fig:instances_num}
%     \end{subfigure}
%     \caption{Visualizations of instance redundancy for (a) sampling percentage and (b) sampling number. Notably, each data point represents the average of 100 sampling iterations to mitigate the impact of randomness. If the sampling number exceeds the maximum benchmark size, all available instances are utilized. Sampling over 40\% or 700 instances can yield average SRCC values greater than 0.99 (indicating nearly identical rankings), suggesting that there is significant redundancy within the current MLLM benchmark instances.}
%     \label{fig:instances_combined}
%     \vspace{-0.2cm}
% \end{figure*}






% \begin{table*}[t]
%     \centering
%     \caption{Categories of Mathematics Tasks in MathVista, MathVision, MathVersion and DynaMath. MathVision and MathVersion predominantly emphasize serious math tasks. MathVista and DynaMath, on the other hand, incorporate a broader spectrum of tasks beyond serious math, such as Scientific Figure Understanding and Visual Question Answering.}
%     \label{tab: mathcategory}
%     \resizebox{\textwidth}{!}{%
%     \begin{tabular}{cc | cccccccc}
%     \toprule[0.15em]
%         % \multirow{2}{*}{Benchmark} & \multirow{2}{*}{Number} & Geometric\&Graph & Numerical Value & Function Type & Math Logic & Real-Life Math Problems & Scientific Figure Understanding & Visual Question Answering & Chart/Table/Diagram Question Answering \\
%         \multirow{2}{*}{Benchmark} & \multirow{2}{*}{Number} & Geometric & Numerical & Function & Math & Real-Life & Scientific Figure & Visual Question & Chart/Table/Diagram \\
%         & & \&Graph & Value &Type &Logic &Math Problems &Understanding &Answering &  Question Answering \\
%         \midrule
%         MathVista & 1k & \checkmark & \checkmark & \checkmark& \checkmark& \checkmark& \checkmark& \checkmark& \checkmark\\
%         MathVision & 3.04k & \checkmark & $\times$ & \checkmark & $\times$ & \checkmark & $\times$& $\times$& $\times$ \\
%         MathVersion & 3.94k & \checkmark & \checkmark & $\times$ & \checkmark & \checkmark & $\times$ & $\times$ & $\times$ \\
%         DynaMath & 501 & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark & $\times$ & $\times$ \\
%     \bottomrule[0.15em]
%     \end{tabular}
%     }%
%     \vspace{-0.2cm}
% \end{table*}







\subsection{Exploration Instance Redundancy}

We include the evaluation results from 18 publicly  available benchmarks in VLMEvalKit~\cite{duan2024vlmevalkit} in our experiments, 
with the average performance across benchmarks presented in \cref{fig:instances_overall}. 
We adopt a similarity threshold of 0.95 for partitioning\footnote{
Ranks with SRCC and PLCC coefficients exceeding 0.95 are considered nearly identical, with only marginal differences in very few cases \cite{hauke2011comparison}. }, 
This leads to an intriguing conclusion: 
\textbf{a majority of existing MLLM benchmarks exhibit significant redundancy in their instances when ranking both Top-50 and Bottom-50 MLLMs, with at least 50\% of the instances being redundant. } 
This indicates that many benchmarks could reduce their instance counts by half without significantly affecting the ranking of MLLMs being tested.
The R² score provides further insight, as it measures how effectively the final performance of MLLMs can be predicted using sampled instances. 
Compared to ensuring accurate ranking, achieving high accuracy in predicting the absolute performance of MLLMs requires a much larger number of instances. 
For example, both Top-50 and Bottom-50 MLLMs require over 90\% of the instances to achieve an R² score greater than 0.95. 
This distinction highlights that fewer instances are sufficient for reliable ranking than for precise performance prediction.

We also compare redundancy tendencies between Top-50 and Bottom-50 MLLMs, 
as shown in \cref{fig:instances_top50,fig:instances_back50}. 
Notably, at the same 0.95 threshold for SRCC and PLCC, 
Bottom-50 MLLMs require significantly fewer instances than Top-50 MLLMs. 
This implies that accurately ranking higher-performing MLLMs (Top-50) demands more instances,
while ranking lower-performing MLLMs (Bottom-50) can be achieved with fewer instances. Consequently, the redundancy of benchmark instances correlates strongly with the capability of the MLLMs being evaluated: \textbf{the stronger the MLLMs, the lower the redundancy of the benchmark instances}.

From the benchmark-specific results (\cref{fig:instances_bench}), 
the redundancy gap between Top-50 and Bottom-50 MLLMs remains consistent across different benchmarks. 
Further examination reveals considerable variation in redundancy levels between benchmarks. For example, in the Top-50 redundancy analysis, 
RealWorldQA~\cite{RealWorldQA} demonstrates relatively low redundancy, 
requiring nearly 80\% of the instances to reach saturation, 
while other benchmarks require far fewer. 
However, for Bottom-50 MLLMs, redundancy levels across benchmarks increase significantly, and the differences between them narrow. 
This illustrates that benchmark redundancy is more prominent when evaluating less capable MLLMs.

It is important to note that the conclusions above are based on the statistical analysis of mainstream benchmarks. 
Specialized benchmarks, with unique design goals or tasks, require case-by-case analyses to assess their instance redundancy accurately. 
Therefore, while these results provide general insights into redundancy trends for standard benchmarks, further evaluation is necessary for niche or task-specific benchmarks.



\subsection{Exploring Cross-Benchmark Redundancy}
To analyze cross-benchmark redundancy, we focus on the Math domain, 
specifically examining several popular mathematical benchmarks:
MathVista~\cite{lu2023mathvista}, MathVision~\cite{zhang2025mathverse}, MathVerse~\cite{wang2024measuring}, and DynaMath~\cite{zou2024dynamath}. 
We utilize the available evaluation results of 37 MLLMs listed on the OpenCompass Reasoning Leaderboard\footnote{\url{https://huggingface.co/spaces/opencompass/Open_LMM_Reasoning_Leaderboard}} and assess their ranking performance across these math benchmarks.
The corresponding heatmap is presented in \cref{fig:math_heatmap}.
The results reveal that, although all four benchmarks are designed to evaluate the mathematical abilities of MLLMs, 
the correlations between them are not particularly strong. 
Among them, MathVista~\cite{lu2023mathvista} exhibits the least redundancy, 
showing the lowest correlation with the other benchmarks. 
In contrast, MathVerse and MathVision demonstrate high redundancy, 
indicating strong correlation with other benchmarks. 
These differences suggest varying levels of overlap in their evaluation focus areas.


To better understand the variability across benchmarks, we analyzed their task distributions. 
While MathVerse and MathVision are exclusively focused on standard mathematical tasks, 
resulting in the highest correlation and substantial overlap with other benchmarks, 
MathVista includes 30\%-40\% of questions outside traditional mathematics, 
such as tasks related to \textit{Scientific Figure Understanding}, \textit{General VQA}, and \textit{Chart/Table/Diagram QA} (see \cref{fig:append_mathvista}(a)(b)(c) for examples). 
As discussed in \cref{sec2.3}, 
low redundancy can arise from unique elements specific to a domain or from irrelevant tasks, 
which we consider ``noise" within the dataset. 
For instance, general VQA tasks, while broadly useful, 
have limited relevance to assessing mathematical ability and contribute to this noise.
To quantify the impact, we systematically removed general VQA tasks from MathVista and recalculated its redundancy with other benchmarks. 
After this refinement, the redundancy between MathVista and other mathematical benchmarks significantly increased, 
aligning more closely with their task profiles. 
Additionally, we identified and excluded \textit{CLEVR}-derived questions categorized as \textit{math-targeted vqa} within MathVista, 
which also had limited relevance to mathematical capabilities (examples in \cref{fig:append_mathvista}(d)).
This further increased overlap with specialized mathematical benchmarks, 
demonstrating that removing irrelevant tasks improves alignment and reduces noise.

% From the observations above, we argue that the common tasks, such as Visual Question Answering, are not quite relative to Math Capability. To prove this, we carefully remove the tasks that are categorized as "general-vqa" in MathVista and recompute the results and redundancy with other three benchmarks, the examples are shown in Append.~\ref{}. It's not surprised that the rundundancy of MathVista without 'general-vqa' tasks with other mathematical benchmarks quickly increases, which suggest it's more relevant to other mathematical benchmarks after filtering common VQA tasks. Further, we clear the questions extracted from CLEVR Benchmark, which are categorized as 'math-targeted vqa' in MathVista but not quite related to math capability, as shown in Append.~\ref{}. We then observe that the redundancy with other math benchmarks improves further, which reaches a quite high level.



% DynaMath, which encompasses a broad range of mathematical tasks and contains few unrelated tasks like Scientific Figure Understanding, also demonstrates a strong correlation with MathVersion and MathVision. 

% Based on the observations above, we posit that maintaining an appropriate degree of independence within benchmarks of the same vertical domain is crucial. However, when redundancy is too low, it may indicate that the benchmark has diverged from the distribution characteristic of that domain. Consequently, this divergence can lead to a misalignment between the benchmark's evaluation capabilities and the core characteristics of the domain.
\begin{figure}[t]
        \centering
        \includegraphics[width=\linewidth]{figs/srcc_matrix_mathvista_hd.pdf}
        \caption{Cross-benchmark redundancy map. MathVision and MathVersion are more focused on the core domain of mathematics (with relatively higher redundancy across other math benchmarks), making them more suitable for benchmarking the mathematical capabilities of MLLMs in a narrow sense.}
        \label{fig:math_heatmap}
        \vspace{-0.3cm}
\end{figure}

% \textbf{Based on the observations above, we argue that the core capabilities of models evaluated across benchmarks within the same vertical domain should be relatively consistent.} When redundancy is excessively low, it may suggest that the benchmark has deviated from the typical distribution of the domain. Such deviation can result in the benchmark's evaluation capabilities no longer accurately reflecting the central characteristics and requirements of the domain.
% From the perspective of redundancy, MathVision and MathVersion share a focus on the core domain of mathematics (with relatively higher redundancy across other math benchmarks), making them particularly suitable for benchmarking the mathematical capabilities of MLLMs in a narrow sense.
% This indirectly demonstrates that our cross-benchmark redundancy approach can effectively identify benchmarks that are not highly focused, while also helping to select those that are more concentrated on specific vertical domains.
% Based on the observations above, we argue that:
% (1) If a in-domain benchmark is targetted on generally evaluating the performance of models within the domain, the redundancy with other benchmarks should be relatively high to show general overlap of a various of sub-capability.
% (2) In contrast, if a benchmark mainly focuses on a small orientation of the domain, the redundancy shall be quite low with other benchmarks, to evaluate the distinct capability of this domain.

Based on these findings, we propose the following principles for benchmark design within a domain:

\begin{itemize}
\item A benchmark intended to broadly assess model performance in one domain should demonstrate relatively high redundancy with other in-domain benchmarks, 
reflecting comprehensive coverage of diverse sub-capabilities and enabling holistic model evaluation.
\item A specialized benchmark should display lower redundancy with other benchmarks, 
focusing on distinct capabilities to fill the vacancy, complement broader assessments, and provide a unique perspective on specific topics in a domain.
\end{itemize}


% A specialized benchmark focusing on distinct topics in the domain (to fill the vacancy) should exhibit significantly lower redundancy with other benchmarks. This reduced overlap ensures that the benchmark evaluates distinct capabilities unique to its focus area, thereby offering a specialized assessment that complements rather than duplicates more general evaluations.


==> sec/4_principle.tex <==

\section{Redundancy Practice Recommendations}

To ensure benchmarks are reliable and efficient, 
we recommend incorporating redundancy detection into the benchmark design process after its initial testing on a set of MLLMs. 
This critical step identifies potential redundancies across dimensions/instances/cross-benchmark overlaps, leading to more precise and meaningful evaluations.

\noindent
\textbf{Dimension Redundancy Check. }
Calculate the dimensional redundancy within the benchmark, 
with particular attention to dimensions exhibiting overall high redundancy. 
Analyze the redundancy heatmap to identify pairs of dimensions with exceptionally strong correlations, 
as these may indicate overlapping capabilities being assessed. 
For such cases, evaluate whether these dimensions are truly necessary or whether they assess similar or redundant skills.

\noindent
\textbf{Instance Redundancy Check. }
Compute the instance redundancy curve to determine whether a smaller subset of benchmark instances can produce results comparable to the full instance set. 
If significant instance redundancy is identified, 
the benchmark should be reviewed, and redundant instances should be reduced. 
This not only streamlines the evaluation process but also optimizes resource usage without compromising the accuracy of results.

\noindent
\textbf{Cross-benchmark Redundancy Check. }
If the benchmark is intended to serve as a representative for a specific domain, 
measure its cross-benchmark redundancy relative to other benchmarks within the domain. 
Higher redundancy indicates stronger representativeness, 
making it a reliable choice for tasks requiring domain coverage. 
Conversely, if the goal is to fill a vacancy in the specific domain (\textit{e.g.}, focusing on a specific topic in mathematics that is not covered by previous benchmarks)
maintaining low redundancy is a more favorable choice.
For use cases focusing on core capabilities within a specific domain under limited resources, 
it is recommended to select the benchmark with the highest cross-benchmark redundancy. 
This ensures that the benchmark comprehensively covers the essential skills while minimizing unnecessary overlaps.


\section{Conclusion}

In conclusion, this paper addresses the pervasive issue of redundancy in MLLM benchmarks, 
impacting both the effectiveness and efficiency of model evaluation. 
We identify redundancy at three levels: dimension, instance, and cross-benchmark redundancy,
and propose a framework with actionable guidelines to improve benchmark design. 
By promoting independence of dimensions, optimizing instance counts, and ensuring purposeful redundancy within specific domains, 
our framework streamlines evaluations and enhances reliability. 
Case studies further demonstrate its utility in refining current practices, 
paving the way for more efficient and accurate MLLM assessments.



% This work underscores the importance of thoughtful benchmark construction in fostering a more effective evaluation ecosystem for MLLMs.

==> sec/XX_finalcopy.tex <==
\section{Final copy}

You must include your signed IEEE copyright release form when you submit your finished paper.
We MUST have this form before your paper can be published in the proceedings.

Please direct any questions to the production editor in charge of these proceedings at the IEEE Computer Society Press:
\url{https://www.computer.org/about/contact}.

==> sec/XX_formatting.tex <==
\section{Formatting your paper}
\label{sec:formatting}

All text must be in a two-column format.
The total allowable size of the text area is $6\frac78$ inches (17.46 cm) wide by $8\frac78$ inches (22.54 cm) high.
Columns are to be $3\frac14$ inches (8.25 cm) wide, with a $\frac{5}{16}$ inch (0.8 cm) space between them.
The main title (on the first page) should begin 1 inch (2.54 cm) from the top edge of the page.
The second and following pages should begin 1 inch (2.54 cm) from the top edge.
On all pages, the bottom margin should be $1\frac{1}{8}$ inches (2.86 cm) from the bottom edge of the page for $8.5 \times 11$-inch paper;
for A4 paper, approximately $1\frac{5}{8}$ inches (4.13 cm) from the bottom edge of the
page.

%-------------------------------------------------------------------------
\subsection{Margins and page numbering}

All printed material, including text, illustrations, and charts, must be kept
within a print area $6\frac{7}{8}$ inches (17.46 cm) wide by $8\frac{7}{8}$ inches (22.54 cm)
high.
%
Page numbers should be in the footer, centered and $\frac{3}{4}$ inches from the bottom of the page.
The review version should have page numbers, yet the final version submitted as camera ready should not show any page numbers.
The \LaTeX\ template takes care of this when used properly.



%-------------------------------------------------------------------------
\subsection{Type style and fonts}

Wherever Times is specified, Times Roman may also be used.
If neither is available on your word processor, please use the font closest in
appearance to Times to which you have access.

MAIN TITLE.
Center the title $1\frac{3}{8}$ inches (3.49 cm) from the top edge of the first page.
The title should be in Times 14-point, boldface type.
Capitalize the first letter of nouns, pronouns, verbs, adjectives, and adverbs;
do not capitalize articles, coordinate conjunctions, or prepositions (unless the title begins with such a word).
Leave two blank lines after the title.

AUTHOR NAME(s) and AFFILIATION(s) are to be centered beneath the title
and printed in Times 12-point, non-boldface type.
This information is to be followed by two blank lines.

The ABSTRACT and MAIN TEXT are to be in a two-column format.

MAIN TEXT.
Type main text in 10-point Times, single-spaced.
Do NOT use double-spacing.
All paragraphs should be indented 1 pica (approx.~$\frac{1}{6}$ inch or 0.422 cm).
Make sure your text is fully justified---that is, flush left and flush right.
Please do not place any additional blank lines between paragraphs.

Figure and table captions should be 9-point Roman type as in \cref{fig:onecol,fig:short}.
Short captions should be centred.

\noindent Callouts should be 9-point Helvetica, non-boldface type.
Initially capitalize only the first word of section titles and first-, second-, and third-order headings.

FIRST-ORDER HEADINGS.
(For example, {\large \bf 1. Introduction}) should be Times 12-point boldface, initially capitalized, flush left, with one blank line before, and one blank line after.

SECOND-ORDER HEADINGS.
(For example, { \bf 1.1. Database elements}) should be Times 11-point boldface, initially capitalized, flush left, with one blank line before, and one after.
If you require a third-order heading (we discourage it), use 10-point Times, boldface, initially capitalized, flush left, preceded by one blank line, followed by a period and your text on the same line.

%-------------------------------------------------------------------------
\subsection{Footnotes}

Please use footnotes\footnote{This is what a footnote looks like.
It often distracts the reader from the main flow of the argument.} sparingly.
Indeed, try to avoid footnotes altogether and include necessary peripheral observations in the text (within parentheses, if you prefer, as in this sentence).
If you wish to use a footnote, place it at the bottom of the column on the page on which it is referenced.
Use Times 8-point type, single-spaced.


%-------------------------------------------------------------------------
\subsection{Cross-references}

For the benefit of author(s) and readers, please use the
{\small\begin{verbatim}
  \cref{...}
\end{verbatim}}  command for cross-referencing to figures, tables, equations, or sections.
This will automatically insert the appropriate label alongside the cross-reference as in this example:
\begin{quotation}
  To see how our method outperforms previous work, please see \cref{fig:onecol} and \cref{tab:example}.
  It is also possible to refer to multiple targets as once, \eg~to \cref{fig:onecol,fig:short-a}.
  You may also return to \cref{sec:formatting} or look at \cref{eq:also-important}.
\end{quotation}
If you do not wish to abbreviate the label, for example at the beginning of the sentence, you can use the
{\small\begin{verbatim}
  \Cref{...}
\end{verbatim}}
command. Here is an example:
\begin{quotation}
  \Cref{fig:onecol} is also quite important.
\end{quotation}

%-------------------------------------------------------------------------
\subsection{References}

List and number all bibliographical references in 9-point Times, single-spaced, at the end of your paper.
When referenced in the text, enclose the citation number in square brackets, for
example~\cite{Authors14}.
Where appropriate, include page numbers and the name(s) of editors of referenced books.
When you cite multiple papers at once, please make sure that you cite them in numerical order like this \cite{Alpher02,Alpher03,Alpher05,Authors14b,Authors14}.
If you use the template as advised, this will be taken care of automatically.

\begin{table}
  \centering
  \caption{\label{tab:example}%
    Results.
    Ours is better.
  }
  \begin{tabular}{lc}
    \toprule
    Method & Frobnability \\
    \midrule
    Theirs & Frumpy \\
    Yours & Frobbly \\
    Ours & Makes one's heart Frob\\
    \bottomrule
  \end{tabular}
\end{table}

%-------------------------------------------------------------------------
\subsection{Illustrations, graphs, and photographs}

All graphics should be centered.
In \LaTeX, avoid using the \texttt{center} environment for this purpose, as this adds potentially unwanted whitespace.
Instead use
{\small\begin{verbatim}
  \centering
\end{verbatim}}
at the beginning of your figure.
Please ensure that any point you wish to make is resolvable in a printed copy of the paper.
Resize fonts in figures to match the font in the body text, and choose line widths that render effectively in print.
Readers (and reviewers), even of an electronic copy, may choose to print your paper in order to read it.
You cannot insist that they do otherwise, and therefore must not assume that they can zoom in to see tiny details on a graphic.

When placing figures in \LaTeX, it's almost always best to use \verb+\includegraphics+, and to specify the figure width as a multiple of the line width as in the example below
{\small\begin{verbatim}
   \usepackage{graphicx} ...
   \includegraphics[width=0.8\linewidth]
                   {myfile.pdf}
\end{verbatim}
}


%-------------------------------------------------------------------------
\subsection{Color}

Please refer to the author guidelines on the \confName\ \confYear\ web page for a discussion of the use of color in your document.

If you use color in your plots, please keep in mind that a significant subset of reviewers and readers may have a color vision deficiency; red-green blindness is the most frequent kind.
Hence avoid relying only on color as the discriminative feature in plots (such as red \vs green lines), but add a second discriminative feature to ease disambiguation.

==> sec/related_work.tex <==
Model Evaluation has always played a crucial role in the development of Multimodal Large Language Models (MLLMs). 
Benchmarks serve not only as tools for assessing model accuracy but also as catalysts for driving innovation and improvements within the field. 
In recent years, with the rapid advancement of MLLMs, there has been an explosive growth in Visual Question Answering (VQA) Benchmarks. 

In the early stages, traditional model evaluation benchmarks such as GQA~\cite{}, VQA-V2~\cite{}, VizWiz~\cite{}, and TextVQA~\cite{} were characterized by relatively simple questions and answers, with responses often being a single word. 
This simplicity imposed significant limitations on the evaluation process. 
The benchmarks were less capable of thoroughly assessing the models' deeper understanding of complex visual scenes or nuanced queries, thereby restricting the scope and depth of performance evaluation.

With the emergence of more powerful MLLMs~\cite{} based on the LLaVA~\cite{} paradigm, traditional evaluation frameworks have become inadequate to meet the flexible evaluation requirements of these advanced models. 
In response, a new generation of VQA benchmarks has arisen, represented by MMBench~\cite{}, MMVet~\cite{}, and MMMU~\cite{}, among others. 
These benchmarks primarily feature multiple-choice questions, offering a more flexible evaluation approach that can better accommodate the complex reasoning and multimodal understanding capabilities of modern MLLMs.

As Multimodal Large Language Models (MLLMs) have rapidly iterated and evolved, their diverse capabilities across various domains have garnered increasing attention. 
This expansion has led to the development of specialized benchmarks tailored to evaluate MLLMs' performance in specific areas:

For \textit{General Understanding}, benchmarks such as MME~\cite{}, SEEDBench~\cite{}, REALworldQA~\cite{}, BLINK~\cite{}, and MMStar~\cite{} have been developed to assess MLLMs' general understanding capabilities, including their ability to comprehend complex contexts, reason about real-world scenarios, and integrate knowledge from different sources. 
In \textit{Mathematics Task}, benchmarks such as MathVista~\cite{}, MathVerse~\cite{}, MathVision~\cite{}, and Dynamath~\cite{} challenge MLLMs with mathematical problems, requiring them to demonstrate not only numerical computation but also conceptual understanding and problem-solving skills. 
For \textit{Optical Character Recognition (OCR)}, benchmarks like OCR-VQA~\cite{}, OCRBench~\cite{}, and DOC-VQA~\cite{} have emerged. These focus on evaluating MLLMs' proficiency in recognizing and interpreting text within images or documents, a critical skill for applications ranging from document processing to assistive technologies. 
\textit{Video Understanding} benchmarks like MV-Bench~\cite{}, MMBench-Video~\cite{}, and VideoMME~\cite{} are designed to test MLLMs' capacity to understand and reason about dynamic visual content.
Moreover, specialized benchmarks have also arisen in Medical Field~\cite{}, Remote Sensing~\cite{}, Agents~\cite{} and GUIs~\cite{}.


Indeed, the explosive growth in the number of benchmarks has inevitably led to overlaps in the capabilities they assess and redundancies among the questions within and across benchmarks. This phenomenon can result in inefficiencies in model evaluation, where similar aspects of MLLM performance are repeatedly tested without adding substantial new insights. Moreover, it can lead to an overemphasis on certain types of tasks while neglecting others, potentially skewing research priorities. In this research, we will delve into this issue with a detailed exploration.
